Not a COINcidence: Sub-Quadratic Asynchronous Byzantine Agreement WHP

King and Saia were the first to break the quadratic word complexity bound for Byzantine Agreement in synchronous systems against an adaptive adversary, and Algorand broke this bound with near-optimal resilience (first in the synchronous model and then with eventual-synchrony). Yet the question of asynchronous sub-quadratic Byzantine Agreement remained open. To the best of our knowledge, we are the first to answer this question in the affirmative. A key component of our solution is a shared coin algorithm based on a VRF. A second essential ingredient is VRF-based committee sampling, which we formalize and utilize in the asynchronous model for the first time. Our algorithms work against a delayed-adaptive adversary, which cannot perform after-the-fact removals but has full control of Byzantine processes and full information about communication in earlier rounds. Using committee sampling and our shared coin, we solve Byzantine Agreement with high probability, with a word complexity of $\widetilde{O}(n)$ and $O(1)$ expected time, breaking the $O(n^2)$ bit barrier for asynchronous Byzantine Agreement.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> sections/consensus_proofs.tex <==


% \begin{lemma}{(Validity)}
% \label{validity}
% If at the beginning of phase $r$ all correct processes have the same estimate value $v$, then any correct process that has not decided before decides $v$ by the end of phase $r$.
% \end{lemma}
% \begin{proof}
% If all correct processes starts phase $r$ with the same estimate value $v$, they all execute ratify($v$). Hence, by ratifier's validity and termination, they all return the non-empty set $\{v\}$ and update their $propose$ value to $v$. Then, they all execute ratify($v$) for the second time and due to the same reason they all return $\{v\}$. By the protocol, any correct process that has not decided before decides $v$ at line 13.
% \end{proof}

% \begin{lemma}{(Agreement)}
% \label{agreement}
% No two correct processes decide different values.
% \end{lemma}
% \begin{proof}
% Let $r$ be the first phase in which a process $p_1$ decides on some value $v$. Thus, $p_1$'s invocation to ratifier in line $9$ of phase $r$ returns $\{v\}$ for $v\neq \bot$. If another correct process $p_2$ also decides in phase $r$ then its ratifier call in line $9$ of phase $r$ returns $\{w\neq \bot\}$. By ratifier's graded agreement $v=w$.
% Consider a correct process $p_3$ that does not decide in phase $r$. By the definition of $r$, $p_3$ hasn't decided in any phase $r'<r$. By ratifier's graded agreement, $p_3$ returns $\{v,\bot\}$ in line $9$ of phase $r$. Thus, $p_3$ updates its $est_p$ value to $v$ in line 18.
% It follows that all correct processes have $v$ as their estimate value in the beginning of phase $r+1$. By Lemma \ref{validity} every correct process that has not decided in phase $r$ decides $v$ in phase $r+1$.
% \end{proof}


% \begin{lemma}
% \label{liveness}
% No correct process remains blocked forever during a phase $r$.
% \end{lemma}
% \begin{proof}
% \shir{still not sure about this proof}

% We show by induction on the phase number $r$ that if all correct process start executing phase $r$, then they all proceeds to phase $r+1$.

% The basis is $r=0$
% The only waits in the protocol is while executing the ratifier and the shared coin primitives (in lines 4,8,9). If all correct process invoke the shared coin and ratifier primitives then their termination property hold and they all return from the call. Thus, since all correct processes start executing the same code in phase $0$, they all return in line 4. Then, they all return in line 8 and in line 9, and proceed to phase $1$.

% Suppose the claim is true for phase $r-1\geq 0$. Thus, if all correct process start executing phase $r-1$ they all proceed to phase $r$. The same reasoning as in the basis applies for phase $r$ and all correct processes proceed to phase $r+1$.

% Therefore, no correct process remains blocked forever during a phase $r$.
% \end{proof}


% \begin{lemma}
% \label{termination}
% Every correct process decides with probability 1.
% \end{lemma}
% \begin{proof}
% Consider phase $r$ of the protocol. By Lemma \ref{liveness} all correct process
% reaches phase $r$ and executes it fully. 
% We examine all possible scenarios in phase $r$:
% \begin{enumerate}
%     \item All correct processes return $\{v\}$ in line 4:
    
%     By ratifier's graded agreement they return $\{v\}$ with the same value $v$. Hence, all correct processes update their $propose$ value to $v$. Then, they all execute ratify($v$) in line 9 and by graded agreement they all return $\{v\}$. By the protocol, they all decide $v$ with probability 1 (if haven't decided yet).
    
%     \item
%     All correct processes return $\{v,\bot\}$ in line 4:
    
%     All correct processes update their $propose$ value to $\bot$. Then,
%     they all execute ratify($\bot$) in line 9 and by graded agreement they  return $\{\bot\}$. By the protocol, all correct processes update their estimate value to the coin toss of the shared coin. With probability $\psi \geq 2\rho$, where $\rho$ is the defiance of the shared coin, all correct processes toss the same $v\in \{0,1\}$. By Lemma \ref{validity}, in phase $r+1$ they all decide $v$ with probability $\psi$ (if haven't decided yet).
%     \shir{we need to mention somewhere that at every phase, the first values that correct processes ratify is indeed 0/1 because we solve binary consensus. otherwise, the coin toss has no meaning. I'm not sure where to mention it}
    
%     % If a correct process decided $v$ before phase $r$, then by Lemma \ref{agreement} no correct process has decided $w\neq v$.
    

    
    
%     \item At least one correct process, but not all correct processes, returns $\{v\}$ in line 4:
    
    
%     We'll examine two possible complementary sub-cases:
    
%     \begin{itemize}
%         \item If a correct process returns $\{v\neq \bot\}$ in line 9:
%         By ratifier's graded agreement no correct process returns $\{\bot\}$ in line 9. Thus, all correct processes update their estimate value to $v$ (in line 11/18). By Lemma \ref{validity}, in phase $r+1$ they all decide $v$ with probability 1 (if haven't decided yet).
        
        
%         \item If no correct process returns $\{v\neq \bot\}$ in line 9:
%         All correct processes either update their estimate value to the coin toss of the shared coin (line 16) or to the same value $v\neq \bot$ (line 18).
%         As the set $props$ contains at most two values, all correct processes that update their value in line 18 update the same value. Since the value $v$ is determined before tossing the coin, the adversary cannot bias $v$ after viewing the coin toss and with probability $\psi \geq \rho$, where $\rho$ is the defiance of the shared coin, all correct processes that adopt the coin's value will toss $v$. By Lemma \ref{validity}, in phase $r+1$ all correct processes decide $v$ with probability $\psi$ (if haven't decided yet).
    
    
%     \end{itemize}

    
% \end{enumerate}

% In all cases, with probability greater than $\rho$ all correct processes decide by phase $r+1$. The probability of not terminating is $\lim_{r\to\infty} (1-\rho)^r$, which equals 0 using our shared coin.	

% \end{proof}


\begin{theorem}
 Algorithm~\ref{alg:consensus_protocol}
solves randomized byzantine binary consensus.
\end{theorem}


\begin{proof}

If all correct processes start with value $v$ then, by Lemma \ref{validity}, they all decide $v$ and validity holds. Agreement follows from Lemma \ref{agreement} and termination follows from Lemma \ref{termination}.

% \begin{description}
% \item[] We show that the protocol satisfies the validity, agreement, and termination properties:
%   \item[Validity]
%   If all correct processes start with value $v$ then, by Lemma \ref{validity}, they all decide $v$.
%   \item[Agreement]
%   Follows from Lemma \ref{agreement}.
%   \item[Termination]
%   Follows from Lemma \ref{termination}.
% \end{description}
\end{proof}

==> sections/ratifier_proofs.tex <==




\begin{lemma}{(Validity)}
\label{rat_validity}
If all correct processes invoke $ratify(v)$ then the only possible return value of correct processes is $\{v\}$.
\end{lemma}
\begin{proof}
Since the number of Byzantine processes is at most $t$, no process receives more than $t$ messages with a value $w\neq v$. Thus, no correct process echoes $\lr{w}$ in line 4. As a result, no $\lr{approve,w}$ message is sent by any correct process. Since $validate(M_{received,v})$ returns \emph{true} only if $2t+1$ processes receive $\lr{v}$, no Byzantine process can send a $\lr{approve,w}$ such that $w$ is validated by a correct process either. Therefore, the only validated value in line 10 is $v$, and no other value is returned.
\end{proof}

\begin{lemma}{(Graded Agreement)}
\label{rat_graded_agreement}
If a correct process $p_1$ returns $\{v\}$ and another correct process $p_2$ returns $\{w\}$ then $v=w$.
\end{lemma}
\begin{proof}
By the protocol, $p_1$ receives $n-t$ $\lr{approve,v}$ messages and $p_2$ receives $n-t$ $\lr{approve,w}$ messages. Since $n\geq 3t+1$ two sets of processes of size $n-t$ intersect by at least $t+1$ processes. Hence, there is at least one correct process $p_3$ whose approve message is received by both $p_1$ and $p_2$. It follows that $p_3$ sent $\lr{approve,v}$ and $\lr{approve,w}$. Since every correct process sends at most one approve message (line 8), $v=w$.

\end{proof}



\begin{lemma}{(Termination)}
\label{rat_termination}
If all correct processes invoke ratifier then every correct process returns with a non-empty set.
\end{lemma}
\begin{proof}
Every correct process sends $\lr{v_i}$ in line 1. Therefore, every correct process receives $n-t>2t+1$ $\lr{v}$ messages. Since correct processes may send two different initial values, one of them is sent by at least $t+1$ processes in line 1. Thus, every correct process receives this value from $t+1$ processes and sends it to all other processes (if it didn't it send it before). As a result, every correct process $p$ receives $2t+1$ $\lr{v}$ messages with the same value $v$, if at this point $p$ have not yet sent $\lr{approve,*}$ message, it sends one. Since there are at least $n-t$ correct processes and they all send \emph{approve} messages, every correct process receives $n-t$ \emph{approve} messages. In addition, because a correct process sends $\lr{approve,v}$ message after it receives $2t+1$, every correct process receives at least $t+1$ $\lr{v}$ messages and thus $v$ is echoed by all correct processes. Therefore, every correct process validates $n-t$ messages and returns the non-empty set of approved values.
\end{proof}


\begin{theorem}
Algorithm \ref{alg:ratifier} implements a ratifier.
\end{theorem}
\begin{proof}
Validity follows from Lemma \ref{rat_validity}, graded agreement follows from Lemma \ref{rat_graded_agreement} and termination follows from Lemma \ref{rat_termination}.
\end{proof}



==> sections/ratifier_protocol.tex <==


\begin{algorithm}
\caption{The ratifier protocol: code for processor $p_i$} 
\begin{algorithmic}[1]

\Statex \textbf{Local variables initialization:}

\State $M_{received} \gets \{\}$; $M_{approved} \gets \{\}$

\Statex

\State send $\lr{v_i}$ to all processes

\Receiving{$\lr{v}$ from process $p_j$}
\State $M_{received} \gets M_{received} \cup \{\lr{j,v}\}$
\If{received $\lr{v}$ from $t+1$ different processes and haven't sent $\lr{v}$ before}
	\State send $\lr{v}$ to all processes
\EndIf
\If{received $\lr{v}$ from $2t+1$ different processes  and haven't sent any $\lr{approve,*}$ message}
	\State send $\lr{approve,v}$ to all processes
\EndIf
\EndReceiving
\Statex



\Receiving{$\lr{approve,v}$ from process $p_j$}
\If{$validate(M_{received}, v)$}
    
	    \State $M_{approved} \gets M_{approved} \cup \{\lr{j,v}\}$
    
    \If{$|M_{approved}|=n-t$}
    	
        % \State let $vals$ be the set of values received in these messages
        \State return $\{v | \lr{j,v}\in M_{approved}\}$
    \EndIf
		

\EndIf
\EndReceiving


% \State wait for $n-t$ \emph{approve} messages 
% \State let $vals$ be the set of values received in these messages
% \If{$|vals|=1$}
% \State return ($commit,v$) where $v$ is the only value in $vals$
% \EndIf
% \State \textbf{otherwise,}  return $(abort,vals$)
% \Statex

% \Receiving{$``approve,v"$ for the first time from $p_j$}
% \State $M_{adopt} \gets M_{adopt} \cup \{\lr{j,v_j}\}$
% \If{$ \exists v \text{ s.t. } |\{j \mid \lr{j,v} \in
% M_{adopt}\}| \geq 2t+1 $}
%         \State   approve $v$
% \EndIf
% \EndReceiving


\end{algorithmic}
\label{alg:ratifier}
\end{algorithm}






\begin{algorithm}
\caption{The validate protocol(set, value):} 
\begin{algorithmic}[1]

\If{$ |\{j \mid \lr{j,value} \in
		set\}| = 2t+1 $ }
\State return \emph{true}
\Else
\State return \emph{false}
\EndIf

\end{algorithmic}
\label{alg:ratifier_validation}
\end{algorithm}






